OmAgent: A Multi-modal Agent Framework for Complex Video Understanding with Task Divide-and-Conquer

Recent advancements in Large Language Models (LLMs) have expanded their capabilities to multimodal contexts, including comprehensive video understanding. However, processing extensive videos such as 24-hour CCTV footage or full-length films presents significant challenges due to the vast data and processing demands. Traditional methods, like extracting key frames or converting frames to text, often result in substantial information loss. To address these shortcomings, we develop OmAgent, efficiently stores and retrieves relevant video frames for specific queries, preserving the detailed content of videos. Additionally, it features an Divide-and-Conquer Loop capable of autonomous reasoning, dynamically invoking APIs and tools to enhance query processing and accuracy. This approach ensures robust video understanding, significantly reducing information loss. Experimental results affirm OmAgent's efficacy in handling various types of videos and complex tasks. Moreover, we have endowed it with greater autonomy and a robust tool-calling system, enabling it to accomplish even more intricate tasks.

==> apx.tex <==
\section{Case Study}
\label{sec:appendix}
In this section, we will illustrate the process by which OmAgent addresses complex video understanding problems through several examples. The primary aspects showcased include: scene caption, inner steps, and agent output. The scene caption displays sample data stored in the knowledge database after the video2RAG preprocessing; the inner steps reveal the task decomposition and execution within the DnC Loop; the agent output presents the final results produced by OmAgent.
